Panchromatic study of star clusters: binaries, blue lurkers, blue stragglers and membership

Binary systems can evolve into immensely different exotic systems such as blue straggle stars (BSSs), yellow straggler stars, cataclysmic variables, type Ia supernovae depending on their initial mass, the orbital parameters and evolution. The aim of this thesis is to understand the demographics of post-mass-transfer systems (BSSs, white dwarfs and blue lurkers) present in the open clusters and how they are formed. First, we identified the cluster members using Gaia EDR3 data in six open clusters. Two of the clusters, M67 and King2, were studied in detail using UVIT, Gaia, GALEX, 2MASS and other archival photometric data. The comprehensive panchromatic study showed that (i) there is a robust mass-transfer pathway for BSSs, and blue lurkers in M67, (ii) at least 15% of BSSs in King 2 were formed via binary mass transfer. We also created a homogeneous catalogue of open cluster BSSs using Gaia DR2 data. The analysis of 868 BSSs across 208 clusters showed that (i) BSS frequency increases with age, (ii) there is a power-law relation between cluster mass and maximum number of BSSs, (iii) the formation mechanism of BSSs is dominated by binary mass transfer (54-67%) though there exists a 10-16% chance of BSSs forming through more than 2 stellar interactions. This study demonstrates that there exists an extensive variety in the demographics of binary products, and the UV observations are vital for their detection and characterisation.

==> certificate.tex <==
\begin{certificate}
This is to certify that the work reported in this doctoral thesis titled ``Panchromatic study of star clusters: binaries, blue lurkers, blue stragglers and membership'' is entirely original and is the result of
investigations carried out by Mr. Vikrant Vinayak Jadhav, Department of Physics, Indian Institute of Science,
Bangalore, under my supervision.

This work has not formed the basis for the award of any degree, diploma, fellowship, associateship or similar title of any University or Institution.


\vspace{2 cm}
\flushleft
Date:\hspace{8 cm}Annapurni Subramaniam\\
%\@degreedate{}
%\flushleft
Bangalore, India\hspace{6 cm} (Supervisor)\\
\hspace{8.9 cm }Indian Institute of Astrophysics\\
%Bangalore, India\hspace{8 cm}~~~~~~~\\
%\@degreedate{}\\
\vfill
\end{certificate}


==> preamble.tex <==
% ******************************************************************************
% ****************************** Custom Margin *********************************

% Add `custommargin' in the document class options to use this section
% Set {innerside margin / outerside margin / topmargin / bottom margin}  and
% other page dimensions
\ifsetCustomMargin
  \RequirePackage[left=37mm,right=30mm,top=35mm,bottom=30mm]{geometry}
  \setFancyHdr % To apply fancy header after geometry package is loaded
\fi

% *****************************************************************************
% ******************* Fonts (like different typewriter fonts etc.)*************

% Add `customfont' in the document class option to use this section

\ifsetCustomFont
  % Set your custom font here and use `customfont' in options. Leave empty to
  % load computer modern font (default LaTeX font).
  \RequirePackage{helvet}
\fi

% *****************************************************************************
% **************************** Custom Packages ********************************

% ************************* Algorithms and Pseudocode **************************

%\usepackage{algpseudocode}


% ********************Captions and Hyperreferencing / URL **********************

% Captions: This makes captions of figures use a boldfaced small font.
%\RequirePackage[small,bf]{caption}

%-----------to make chapter heading fancy--------------------------
%.......... added by prasun/Vikrant .........%
\usepackage{adjustbox}
\usepackage{afterpage}
\usepackage{amsbsy}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}	% Extra maths symbols
\usepackage{array}
\usepackage{booktabs} % For professional looking tables
\usepackage{bm}
\usepackage{cool}
\usepackage{deluxetable}
\usepackage{enumitem}
% \usepackage{epsfig}
% \usepackage{epstopdf}
\usepackage{graphicx}	% Including figure files
\usepackage{longtable}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{pdflscape}
\usepackage[grey]{quotchap}
\usepackage{rotating}
\usepackage{siunitx} % use this package module for SI units
\usepackage{soul}
\usepackage{textcomp}
\usepackage{tikz}
\usepackage{wrapfig}
\usepackage[normalem]{ulem}
\let\captionwidth\relax
\usepackage{ccaption}
\usepackage{caption}
\captionsetup{margin=10pt,font=small,labelfont=bf}
% \usepackage{layouts}  % for printin   g \textwidth ~ 15.7 cm here

% Subcaption package is also available in the sty folder you can use that by
% uncommenting the following line
% This is for people stuck with older versions of texlive
%\usepackage{sty/caption/subcaption}
% \usepackage{subcaption}

%\usepackage{multicol}
%\usepackage{longtable}
%\usepackage{tabularx}

%\usepackage{mathabx}
%\usepackage{gensymb}
%\qsetcnfont{lmr}

\makeatletter
\renewcommand\chapter{%
  \if@openright\cleardoublepage\else\clearpage\fi
  \thispagestyle{plain}%
  \global\@topnum\z@
%   \@printcites% DELETED
  \null\hfill\@printcites\par% NEW
  \@afterindentfalse
  \secdef\@chapter\@schapter
}
\renewcommand{\@makechapterhead}[1]{%
  \chapterheadstartvskip%
%   {\size@chapter{\sectfont\raggedleft% DELETED
  {\size@chapter{\sectfont\raggedright% NEW
    {\chapnumfont
      \ifnum \c@secnumdepth >\m@ne%
      \if@mainmatter\thechapter%
      \fi\fi
      \par\nobreak}%
%     {\raggedleft\advance\leftmargin10em\interlinepenalty\@M #1\par}}% DELETED
    {\raggedright\advance\leftmargin10em\interlinepenalty\@M #1\par}}% NEW
  \nobreak\chapterheadendvskip}}
\makeatother
%----------------fancy chapter style ends------------------------------


\RequirePackage[labelsep=space,tableposition=top]{caption}
\renewcommand{\figurename}{Fig.} %to support older versions of captions.sty




% Uncomment the following two lines to force Latex to place the figure.
% Use [H] when including graphics. Note 'H' instead of 'h'
%\usepackage{float}
%\restylefloat{figure}








% ******************************* Line Spacing *********************************

% Choose linespacing as appropriate. Default is one-half line spacing as per the
% University guidelines

% \doublespacing
% \onehalfspacing
% \singlespacing


% ************************ Formatting / Footnote *******************************

% Don't break enumeration (etc.) across pages in an ugly manner (default 10000)
%\clubpenalty=500
%\widowpenalty=500

%\usepackage[perpage]{footmisc} %Range of footnote options


% *****************************************************************************
% *************************** Bibliography  and References ********************

%\usepackage{cleveref} %Referencing without need to explicitly state fig /table

% Add `custombib' in the document class option to use this section
\ifuseCustomBib
   %\RequirePackage[square, sort, numbers, authoryear]{natbib} % CustomBib
     \RequirePackage[numbers, authoryear]{natbib} % CustomBib
% If you would like to use biblatex for your reference management, as opposed to the default `natbibpackage` pass the option `custombib` in the document class. Comment out the previous line to make sure you don't load the natbib package. Uncomment the following lines and specify the location of references.bib file

%\RequirePackage[backend=biber, style=numeric-comp, citestyle=numeric, sorting=nty, natbib=true]{biblatex}
%\bibliography{References/references} %Location of references.bib only for biblatex

\fi

% changes the default name `Bibliography` -> `References'
\renewcommand{\bibname}{References}


% *****************************************************************************
% *************** Changing the Visual Style of Chapter Headings ***************
% This section on visual style is from https://github.com/cambridge/thesis

% Uncomment the section below. Requires titlesec package.

%\RequirePackage{titlesec}
%\newcommand{\PreContentTitleFormat}{\titleformat{\chapter}[display]{\scshape\Large}
%{\Large\filleft{\chaptertitlename} \Huge\thechapter}
%{1ex}{}
%[\vspace{1ex}\titlerule]}
%\newcommand{\ContentTitleFormat}{\titleformat{\chapter}[display]{\scshape\huge}
%{\Large\filleft{\chaptertitlename} \Huge\thechapter}{1ex}
%{\titlerule\vspace{1ex}\filright}
%[\vspace{1ex}\titlerule]}
%\newcommand{\PostContentTitleFormat}{\PreContentTitleFormat}
%\PreContentTitleFormat


% ******************************************************************************
% ************************* User Defined Commands ******************************
% ******************************************************************************

% *********** To change the name of Table of Contents / LOF and LOT ************

%\renewcommand{\contentsname}{My Table of Contents}
%\renewcommand{\listfigurename}{My List of Figures}
%\renewcommand{\listtablename}{My List of Tables}


% ********************** TOC depth and numbering depth *************************

\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}


% ******************************* Nomenclature *********************************

% To change the name of the Nomenclature section, uncomment the following line

%\renewcommand{\nomname}{Symbols}


% ********************************* Appendix ***********************************

% The default value of both \appendixtocname and \appendixpagename is `Appendices'. These names can all be changed via:

%\renewcommand{\appendixtocname}{List of appendices}
%\renewcommand{\appendixname}{Appndx}

% ******************************** Draft Mode **********************************

% Uncomment to disable figures in `draftmode'
%\setkeys{Gin}{draft=true}  % set draft to false to enable figures in `draft'

% These options are active only during the draft mode
% Default text is "Draft"
%\SetDraftText{DRAFT}

% Default Watermark location is top. Location (top/bottom)
%\SetDraftWMPosition{bottom}

% Draft Version - default is v1.0
%\SetDraftVersion{v1.1}

% Draft Text grayscale value (should be between 0-black and 1-white)
% Default value is 0.75
%\SetDraftGrayScale{0.8}


%% Todo notes functionality
%% Uncomment the following lines to have todonotes.

%\ifsetDraft
%	\usepackage[colorinlistoftodos]{todonotes}
%	\newcommand{\mynote}[1]{\todo[author=kks32,size=\small,inline,color=green!40]{#1}}
%\else
%	\newcommand{\mynote}[1]{}
%	\newcommand{\listoftodos}{}
%\fi

% Example todo: \mynote{Hey! I have a note}

\def \be{\begin{equation}}
\def \ee{\end{equation}}
\newcommand       \ba           {\begin{eqnarray}}
\newcommand       \ea           {\end{eqnarray}}
\def \bea{\begin{eqnarray}}
\def \eea{\end{eqnarray}}
\def\etal{{et al.\ }}
\def\et{{\it et al.}}
\def \cb {\textcolor{blue}}
\def \ccr {\textcolor{red}}
\def \ccc{\textcolor{cyan}}
\def \cmag{\textcolor{magenta}}
\newcommand{\angstrom}{\textup{\AA}}
\newcommand\arcdeg{\mbox{$^\circ$}}%
\newcommand\arcmin{\mbox{$^\prime$}}%
\newcommand\arcsec{\mbox{$^{\prime\prime}$}}%
\newcommand\farcdeg{\mbox{$.\!\!^\circ$}}%
\newcommand\farcmin{\mbox{$.\mkern-4mu^\prime$}}%
\newcommand\farcsec{\mbox{$.\!\!^{\prime\prime}$}}%
\newcommand\micron{\mbox{$\mu$m}}%
\newcommand{\Me}{  {$\mathcal{M}_{e}$}}
\newcommand{\Mnom} {{M$_{\odot}$}}
\newcommand{\Msun} {{M$_{\odot}$}}
\newcommand{\Lsun} {{L$_{\odot}$}}
\newcommand{\Rsun} {{R$_{\odot}$}}
\newcommand{\textred} {\textcolor{red}}
\def\bm#1{\mbox{\boldmath $#1$}}
\newcommand{\comments}[1]{}
\newcommand       \grad         {\nabla}
\newcommand   \la          {\langle}
\newcommand       \ra          {\rangle}

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\definecolor{webgreen}{rgb}{0,.5,0}
\definecolor{webbrown}{rgb}{.6,0,0}
%\usepackage[pdfpagelabels]{hyperref}
\hypersetup{%
   colorlinks=true,%hyperfootnotes=false,%
   breaklinks=true,%
   plainpages=false, bookmarksnumbered, bookmarksopen=true,
   bookmarksopenlevel=1,%
   urlcolor=webbrown, linkcolor=webbrown, citecolor=webgreen,
   }

% ...................%

%\usepackage{adjustbox}
%\usepackage{jcappub}

%\usepackage{hyperref}
% ******* Abstract Separate ****************
% To printout only the titlepage and the abstract with the PhD title and the
% author name for submission to the Student Registry, use the `abstract' option in
% the document class.

%\ifdefineAbstract
% \pagestyle{empty}
% \includeonly{declaration, abstract}
%\fi

% *********** Chapter Mode *******************
% The chapter mode allows user to only print particular chapters with references
% Title, Contents, Frontmatter are disabled by default
% Useful option to review a particular chapter or to send it to supervisior.
% To use choose `chapter' option in the document class

%\ifdefineChapter
% \includeonly{chapter3}
%\fi
%adding a footnote without marker
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

